Window Attention is Bugged: How not to Interpolate Position Embeddings

Window attention, position embeddings, and high resolution finetuning are core concepts in the modern transformer era of computer vision. However, we find that naively combining these near ubiquitous components can have a detrimental effect on performance. The issue is simple: interpolating position embeddings while using window attention is wrong. We study two state-of-the-art methods that have these three components, namely Hiera and ViTDet, and find that both do indeed suffer from this bug. To fix it, we introduce a simple absolute window position embedding strategy, which solves the bug outright in Hiera and allows us to increase both speed and performance of the model in ViTDet. We finally combine the two to obtain HieraDet, which achieves 61.7 box mAP on COCO, making it state-of-the-art for models that only use ImageNet-1k pretraining. This all stems from what is essentially a 3 line bug fix, which we name "absolute win".

==> figures/01_hiera_posemb.tex <==
\begin{minipage}{0.48\linewidth}{
    \includegraphics[width=\linewidth]{figures/img/hiera_posemb.png}
    
    \captionof{figure}{\textbf{Abs Pos Embed~for Window Attn.} A channel from the \textit{learned} absolute position embeddings in Hiera \cite{hiera}, a simple hierarchical ViT that uses window attention. }
    \label{fig:hiera_posemb}
}\end{minipage}

==> figures/02_window_sim.tex <==

    \includegraphics[width=\linewidth]{figures/img/window_sim.png}
    
    \captionof{figure}{\textbf{Window Repetition} increases over training for the baseline Hiera models. Here we measure the average pairwise cosine similarity between the position embedding of each window.  }
    \label{fig:window_sim}

==> figures/03_absolute_win.tex <==

    \includegraphics[width=\linewidth]{figures/img/absolute_win.png}
    
    \captionof{figure}{\textbf{Absolute Win} embraces the behavior in Fig.~\ref{fig:hiera_posemb} by explicitly learning position embeddings as the sum of a tiled \textit{window embedding} and an interpolated \textit{global embedding}. See Appendix~\ref{appx:more_embedding_vis} for more learned embedding examples.  }
    \label{fig:absolute_win}

==> figures/04_embed_action.tex <==

    \includegraphics[width=\linewidth]{figures/img/embed_action.png}
    
    \captionof{figure}{\textbf{Absolute Win Similarity.} Cosine similarity between tokens in the learned window and global embeddings (Fig.~\ref{fig:absolute_win}). E.g., the top left patch for window embed compares the top left token in the window embedding with all other tokens in the window embedding.  }
    \label{fig:absolute_win_action}

==> figures/05_hiera_motivation.tex <==
\begin{minipage}{0.48\linewidth}{
    \centering
    \tablestyle{4pt}{1.08}
    \begin{tabular}{y{45}y{48}x{28}x{36}}
        \multicolumn{2}{c}{}       & \multicolumn{2}{c}{in-1k acc @ ft res} \\
        model    & pos embed & 224px & 256px                       \\
        \shline
        Hiera-L$_{\text{MAE}}$ & absolute        & 85.6        & 85.2 \bad{0.4}        \\
        & \baseline{{\bf absolute win}}  & \baseline{\bf 85.7}  & \baseline{\bf 86.0 \good{0.3}} \\
        \hline
        Hiera-B$_{\text{Sup}}$ & absolute & 81.8 & 81.4 \bad{0.4} \\
                   & absolute win & 82.4 &  82.7 \good{0.3} \\
    \end{tabular}
    \captionof{table}{\textbf{Finetuning at higher res} than the default (224px) fails when using a Hiera model with its default absolute pos emb. Absolute win fixes this for MAE trained models and increases performance for fully supervised {(Sup)} models. }
    \label{tab:motivation}
}\end{minipage}

==> figures/06_bkg_size.tex <==

    \centering
    \tablestyle{4pt}{1.08}
    % \begin{tabular}{x{42}|x{24}x{24}x{24}}
    %     & \multicolumn{3}{c}{in-1k acc @ ft res} \\
    %     bkg size & 224px & 256px & diff \\\shline
    %     % $56\times56$ & 85.6 & 85.2 & \textcolor{bad}{-0.4} \\
    %     % $28\times28$ &  &  & \\
    %     $14\times14$ & \textbf{85.7} &      &      \\
    %     \baseline{$7\times7$}   & \baseline{\textbf{85.7}} & \baseline{\textbf{86.0}} & \baseline{\textcolor{good}{+0.3}} \\
    %     % $5\times5$   & 85.6 &      &      \\
    %     $3\times3$   & 85.5 &      &      \\
    %     $1\times1$   & 84.8 & 85.1 & \textcolor{good}{+0.3} \\
    % \end{tabular}
    \begin{tabular}{y{50}x{42}x{28}x{36}}
        \multicolumn{2}{c}{position embedding}       & \multicolumn{2}{c}{in-1k acc @ ft res} \\
        method       & global size  & 224px         & 256px                    \\
        \shline
        \textbf{absolute win} & $14\times14$ & \textbf{85.7} & 85.9 \good{0.2} \\
                     & \baseline{$7\times7$}   &\baseline{\textbf{85.7}} & \baseline{\bf 86.0 \good{0.3}} \\
                     & $3\times3$   & 85.5          & 85.9 \good{0.4}                     \\
        \hline
        global only  & $7\times7$   & 85.5          & 85.8 \good{0.3}          \\
        window only  & none         & 84.8          & 85.1 \good{0.3}          \\
        
    \end{tabular}
    \captionof{table}{\textbf{Varying Global Size.} We default to a global embedding of $7\times7$ for the global embedding in Tab.~\ref{tab:motivation}. This turns out to be optimal for both 224px and 256px acc (Hiera-L$_\text{MAE}$). }
    \label{tab:bkg_size}

==> figures/07_vitdet_motivation.tex <==
\begin{minipage}{0.48\linewidth}{
    \centering
    \tablestyle{4pt}{1.08}
    \begin{tabular}{x{28}x{28}y{36}y{36}x{20}}
           &               & \multicolumn{2}{c}{COCO mAP}                          &               \\
    relpos & abs win       & \multicolumn{1}{c}{box}     & \multicolumn{1}{c}{mask}& ms/im         \\\shline
    all    & \xmark{}      & 55.6                        & 49.2                    & 97            \\
           & \checkmark{}  & {\bf 55.8} \good{0.2}       & 49.3 \good{0.1}         & 97            \\\hline
    none   & \xmark{}      & 54.6                        & 48.5                    & 66            \\
           & \checkmark{}  & 55.0 \good{0.4}             & 49.1 \good{0.6}         & 66            \\\hline
    ga only& \xmark{}      & 55.1                        & 48.9                    & 69            \\
           & \baseline{\checkmark{}}& \baseline{\bf 55.8 \good{0.7}}         & \baseline{\bf 49.6 \good{0.7}}     & \baseline{68} \\
    \end{tabular}
    \captionof{table}{{\bf Fixing ViTDet-L} by tiling the original position embeddings. Absolute win reduces the need for relative position embeddings (relpos) to only the 4 global attention (ga) layers. }
    \label{tab:vitdet_motivation}
}\end{minipage}

==> figures/08_detection_abl.tex <==
\begin{minipage}{0.48\linewidth}{
    \centering
    \tablestyle{4pt}{1.08}
\tablestyle{4pt}{1.08}
\begin{tabular}{y{28}y{44}x{24}x{24}x{20}}
          &                    & \multicolumn{2}{c}{COCO mAP}                         &                \\
strategy  & location           & \multicolumn{1}{c}{box}    & \multicolumn{1}{c}{mask}& ms/im          \\\shline
relative  & all attn           & {\bf 55.8}                 & 49.3                    & 97            \\
          & win attn           & 55.0                       & 49.0                    & 75             \\
          & \baseline{global attn} & \baseline{\bf 55.8}    & \baseline{\bf 49.6}     & \baseline{68} \\\hline
absolute  & patchify           & 55.1                       & 49.1                    & 66              \\
          % & win qkv            &                            &                         &                \\
          & global block       & 55.1                       & 49.0                    & 66             \\
          & global qkv         & 55.0                       & 49.0                    & 67             \\
\end{tabular}
    \captionof{table}{\textbf{Global Embed for ViTDet.} Learning absolute position embeddings from scratch during finetuning doesn't work, so we opt to use relpos added to just global attention instead.  }
    \label{tab:detection_ablations}
}\end{minipage}
% even layers       & 55.0                       & 48.9                    &                \\
% odd layers        & 55.6                       & 49.4                    &                \\
% first half        & 55.4                       & 49.3                    &                \\
% even layers       & 55.6                       & 49.2                    &                \\

==> figures/09_detection_posemb.tex <==
\begin{minipage}{0.48\linewidth}{
    \includegraphics[width=\linewidth]{figures/img/detection_posemb.png}
    
    \captionof{figure}{\textbf{Absolute Win for Detection.} For detection, we apply absolute win \textit{recursively} by tiling the original model's pos embed. }
    \label{fig:detection_posemb}
}\end{minipage}

==> figures/10_hieradet_motivation.tex <==
\begin{minipage}{0.48\linewidth}{
    \centering
    \tablestyle{4pt}{1.08}

\newcommand{\ours}[1]{{#1}$^\ddagger$ }
\begin{tabular}{y{45}x{28}x{28}x{28}x{20}}
                                  &                        & \multicolumn{2}{c}{COCO mAP}                           &                         \\
model                             & abs win                & \multicolumn{1}{c}{box}     & \multicolumn{1}{c}{mask} & ms/im                   \\\shline
\gc{ViT-L}                        & \gc{\xmark{}}          & \gc{55.6}                   & \gc{49.2}                & \gc{97}                \\
\gc{{ViT-L}}                 & \gc{\checkmark{}}      & \gc{55.8}                   & \gc{49.6}                & \gc{68}                \\\hline
Hiera-L                           & \xmark{}               & 55.0                        & 48.6                     & -                     \\

\ours{Hiera-L}                    & \xmark{}               & 55.6                        & 49.3                     & 92                     \\
\baseline{\ours{Hiera-L}}         & \baseline{\checkmark{}}& \baseline{\textbf{56.2}}    & \baseline{\textbf{50.0}} & \baseline{\textbf{67}} \\
\end{tabular}
    \captionof{table}{{\bf Fixing HieraDet-L} by applying absolute win \textit{recursively}. Our implementation ($\ddagger$) already outperforms the original \cite{hiera}, but absolute win embeddings allows HieraDet to considerably outperform even ViTDet. }
    \label{tab:hieradet_motivation}
}\end{minipage}

==> figures/11_imnet_results.tex <==

    \centering
    \tablestyle{4pt}{1.08}

% \begin{tabular}{y{60}x{22}z{22}x{22}z{22}}
%                   & \multicolumn{2}{c|}{224px}        & \multicolumn{2}{c}{384px}  \\  
% model             & top-1          & flops           & top-1      & flops         \\\shline
% Swin-B$^\dagger$  & 83.5           & 15.4G           & 84.5       & 47.0G         \\
% MViTv2-B$^\dagger$& 84.4           & 10.2G           & 85.2       & 36.7G         \\
% Hiera-B           & 84.5           & 9.4G            &            & 30.3G         \\
% \ours{Hiera-B}    & \baseline{84.5}& \baseline{9.4G }& \baseline{85.8}& \baseline{30.3G}   \\
% \ours{Hiera-B+}   & \baseline{85.1}& \baseline{12.7G}& \baseline{86.2}& \baseline{40.3G}   \\\hline
% MViTv2-L$^\dagger$& 85.3           & 42.1G           & 86.0       & 140G        \\
% Hiera-L           & 86.1           & 40.3G           &            & 128G        \\
% \ours{Hiera-L}    & \baseline{86.1}& \baseline{40.3G}& \baseline{86.9}& \baseline{128G}   \\\hline
% Hiera-H           & 86.9           &                 &            &               \\
% \ours{Hiera-H}    & \baseline{86.8}& \baseline{    } & \baseline{}& \baseline{}   \\
% \end{tabular}
\newcommand{\ours}[1]{\baseline{\bf #1}$_{\text{\tiny{abs win}}}$}
\newcommand{\flo}[2][G]{{\textcolor{black}{\scriptsize{#2#1}}}}
\renewcommand{\good}[1]{\textcolor{good}{{+#1}}}
\newcommand{\ehh}[1]{\textcolor{gray}{{+#1}}}
\renewcommand{\bad}[1]{\textcolor{bad}{{-#1}}}

\begin{tabular}{y{56}x{15}z{16}x{15}z{16}x{22}}
    & \multicolumn{2}{c}{224px}             & \multicolumn{2}{c}{384px}              &    $\Delta$                    \\  
model             & acc            & \flo[]{flops}        & acc            & \flo[]{flops}         &     acc                    \\\shline
MViTv2-B$^\dagger$& \underline{84.4}           & \flo{10.2}           & 85.2           & \flo{36.7}            &  \good{0.8}               \\
Hiera-B           & {\bf 84.5}           & \flo{ 9.4}            &   85.0     & \flo{30.3}            &  \good{0.5}                   \\
\ours{Hiera-B}    & \baseline{\bf 84.5}& \flo{ \baseline{9.4}} & \baseline{\bf 85.8}& \flo{\baseline{30.3}} &  \baseline{\bf \good{1.3}}    \\\hline
Swin-B$^\dagger$  & 83.5           & \flo{15.4}           & 84.5           & \flo{47.0}            &  \good{1.0}               \\
Hiera-B+          & {\bf 85.2}           & \flo{12.7}            & 85.2   & \flo{40.3}            &  \ehh{0.0}                   \\
\ours{Hiera-B+}   & \baseline{\underline{85.1}}& \flo{\baseline{12.7}}& \baseline{\bf 86.2}& \flo{\baseline{40.3}} &  \baseline{\bf \good{1.1}}    \\\hline
MViTv2-L$^\dagger$& \underline{85.3}           & \flo{42.1}           & 86.0           & \flo{140}             &  \good{0.7}               \\
Hiera-L           & {\bf 86.1}           & \flo{40.3}           &   86.4         & \flo{128}             &  \good{0.3}                   \\
\ours{Hiera-L}    & \baseline{\bf 86.1}& \flo{\baseline{40.3}}& \baseline{\bf 86.9}& \flo{\baseline{128}}  &  \baseline{\bf \good{0.8}}    \\\hline
Hiera-H           & {\bf 86.9}           & \flo{125}               & 86.7               & \flo{383}                &  \bad{0.2}                   \\
\ours{Hiera-H}    & \baseline{\underline{86.8}}& \flo{\baseline{125}}   & \baseline{\bf 87.3}    & \flo{\baseline{383}}     &  \baseline{\bf \good{0.5}}        \\
\end{tabular}


    \captionof{table}{\textbf{ImageNet-1k Results.} Comparing to other models that train at both 224px and 384px. Hiera with our absolute win gains more from high res than others \cite{mvit2,swin,hiera}. $^\dagger$ Fully supervised. }
    \label{tab:imnet_results}

==> figures/12_imnet_scale.tex <==

    \centering
    \tablestyle{3pt}{1.08}
\newcommand{\ours}{{\bf {\scriptsize{w/}} abs win}}

\begin{tabular}{y{38}x{22}x{34}x{34}x{34}x{34}}
             &           & \multicolumn{3}{c}{in-1k acc @ ft res}                                          \\
model        & 224px     & 256px                    & 320px                    & 448px                     \\\shline
Hiera-B      & 84.5      & 84.2 \bad {0.3}          & 84.6 \good{0.1}          & 84.8 \good{0.3}           \\
\bln{\ours{}}& \bln{84.5}& \bln{\bf 84.9 \good{0.4}}& \bln{\bf 85.4 \good{0.9}}& \bln{\bf 85.7 \good{1.2}} \\\hline
Hiera-B+     & 85.2      & 84.3 \bad {0.9}          & 85.1 \bad{0.1}           & 84.9 \bad{0.3}            \\
\bln{\ours{}}& \bln{85.1}& \bln{\bf 85.3 \good{0.2}}& \bln{\bf 86.0 \good{0.9}}& \bln{\bf 86.2 \good{1.1}} \\\hline
Hiera-L      & 86.1      & 85.7 \bad {0.4}          & 86.2 \good{0.1}          & 86.6 \good{0.5}           \\
\bln{\ours{}}& \bln{86.1}& \bln{\bf 86.5 \good{0.4}}& \bln{\bf 86.7 \good{0.6}}& \bln{\bf 87.0 \good{0.9}} \\\hline
Hiera-H      & 86.9      & 86.5 \bad{0.4}                         &                   86.9 \bad{0.0}    &         86.5 \bad{0.4}          \\
\bln{\ours{}}& \bln{86.8}& \bln{\bf 87.0 \good{0.2} }    & \bln{\bf 87.2 \good{0.4} }               & \bln{\bf 87.3 \good{0.5}}                \\
\end{tabular}


    \captionof{table}{\textbf{Image Size Comparison.} Evaluating the performance of absolute win on additional finetune resolutions. Without absolute win, performance significantly degrades. Note that we use the same hyperparameters in each experiment here, which is not necessarily optimal. % The original Hiera models \textit{do} increase in performance at some resolutions (especially 448, a multiple of 224). However, absolute win outperforms in every case.
    }
    \label{tab:imnet_scale}

==> figures/13_k400_results.tex <==

    \centering
    \tablestyle{4pt}{1.08}
\newcommand{\ours}[1]{\baseline{\bf #1}$_{\text{\tiny{abs win}}}$}
\newcommand{\flo}[2][G]{{\textcolor{black}{\scriptsize{#2#1}}}}

\renewcommand{\good}[1]{\textcolor{good}{{+#1}}}
\renewcommand{\bad}[1]{\textcolor{gray}{{+#1}}}

\begin{tabular}{y{51}x{18}z{18}x{18}z{18}x{18}}
                  & \multicolumn{2}{c}{16$\times$224px}    & \multicolumn{2}{c}{32$\times$320px} & $\Delta$  \\  
model             & acc            & \flo[]{flops}         & acc            & \flo[]{flops}      & acc \\\shline
ViT-L             & 85.2           & \flo{597}             & 86.1           & \flo{3958}         & {\bf \good{0.9}} \\
Hiera-L           & {\bf 87.3}     & \flo{413}             & 87.4           & \flo{2962}             & \good{0.1} \\
\ours{Hiera-L}    & \baseline{\underline{87.1}}& \flo{\baseline{413}}  & \baseline{{\bf 88.0}}& \baseline{\flo{2962}}  &  \baseline{\bf \good{0.9}}\\\hline
ViT-H             & 86.6           & \flo{1192}            & 87.4           & \flo{7397}         & {\bf \good{0.8}} \\
Hiera-H           & {\bf 87.8}     & \flo{1159}            & 88.1           & \flo{7003}             & \good{0.3}  \\
\ours{Hiera-H}    & \baseline{\underline{87.6}}& \flo{\baseline{1159}} & \baseline{{\bf 88.4}}& \baseline{\flo{7003}}  & \bln{\bf \good{0.8}} \\
\end{tabular}

    \captionof{table}{\textbf{Kinetics-400 Results.} Frames $\times$ img size w/ 3 spatial and 5 temporal crops. ViT uses 4 temporal crops at high res \cite{videomae}. }
    \label{tab:k400_results}

==> figures/14_ava_results.tex <==

    \centering
    \tablestyle{4pt}{1.08}
\newcommand{\ours}[1]{\baseline{\bf #1}$_{\text{\tiny{abs win}}}$}
\newcommand{\flo}[2][G]{{\textcolor{black}{\scriptsize{#2#1}}}}

\begin{tabular}{y{52}x{22}x{22}x{22}z{18}}
model         & frames       & size              & mAP        & flops             \\\shline
ViT-L         & 16           & $224^2$           & 37.0       & \flo{597}              \\
{MViTv2-L}    & {40}         & {$312^2$}         & 38.5       & \flo{2828}             \\
Hiera-L       & 16           & $224^2$           & \underline{39.8}       & \flo{413}              \\
\ours{Hiera-L}& \baseline{32}& \baseline{$320^2$}& \baseline{\bf 42.4}& \baseline{\flo{2962}}       \\\hline
ViT-H         & 16           & $224^2$           & 39.5       & \flo{633}              \\
Hiera-H       & 16           & $224^2$           & \underline{42.5}       & \flo{672}              \\
\ours{Hiera-H}& \baseline{32}& \baseline{$320^2$}& \baseline{\bf 43.8}& \baseline{\flo{7003}}       \\
\end{tabular}



    \captionof{table}{\textbf{AVA v2.2 Results.} Video action localization compared to models pretrained on K400 with masked image modeling \cite{videomae,hiera,maskfeats}. }
    \label{tab:ava_results}

==> figures/15_coco_backbones.tex <==

    \centering
    \tablestyle{4pt}{1.08}
\newcommand{\ours}[1]{\baseline{\bf #1}$_{\text{\tiny{abs win}}}$}
\newcommand{\oursb}[1]{\baseline{\bf #1}$^\ddagger$$_{\text{\tiny{abs win}}}$}
\newcommand{\spv}[1]{{#1}$^\dagger$}

\begin{tabular}{y{60}x{22}x{22}x{22}x{22}}
    & \multicolumn{2}{c}{\tiny{Mask R-CNN}} & \multicolumn{2}{c}{\tiny{Cascade Mask R-CNN}} \\
model            & AP$^{\text{box}}$ & AP$^{\text{mask}}$ & AP$^{\text{box}}$ & AP$^{\text{mask}}$ \\\shline
% \spv{Swin-B}     & 51.4 & 45.4 & 54.0 & 46.5 \\
% \spv{MViTv2-B}   & 53.1 & 47.4 & 55.6 & 48.1 \\
{ViT-B}          & 51.6  &  45.9    &  54.0    & 46.7     \\
\ours{ViT-B}     & \baseline{\bf 52.2} & \baseline{\bf 46.2} & \baseline{\bf 54.1} & \baseline{\bf 47.0} \\%\hdashline[8pt/4pt]
{Hiera-B }       & 52.2 & 46.3  &  -   & -    \\
\oursb{Hiera-B}   & \baseline{\bf 53.7} & \baseline{\bf 47.9} & \baseline{\bf 55.8} & \baseline{\bf 48.4} \\%\hdashline[8pt/4pt]
{Hiera-B+}       & 53.5 & 47.3 &  -   & -    \\
\oursb{Hiera-B+} & \baseline{\bf 54.3} & \baseline{\bf 48.2} & \baseline{\bf 56.8} & \baseline{\bf 49.1} \\\hline
% \spv{Swin-L}     & 52.4 & 46.2 & 54.8 & 47.3 \\
% \spv{MViTv2-L}   & 53.6 & 47.5 & 55.7 & 48.3 \\
{ViT-L}       &  55.6    &  49.2    & 57.6    & 49.8    \\
\ours{ViT-L}     & \baseline{\bf 55.8} & \baseline{\bf 49.6} & \baseline{\bf 57.8} & \baseline{\bf 50.0} \\%\hdashline[8pt/4pt]
{Hiera-L}       & 55.0  & 48.6  &  -   & -    \\
\oursb{Hiera-L}   & \baseline{\bf 56.2} & \baseline{\bf 50.0} & \baseline{\bf 58.4} & \baseline{\bf 50.7} \\\hline
% \spv{MViTv2-H}   & 54.1 & 47.7 & 55.8 & 48.3 \\
{ViT-H}       & 56.7     &  50.1    & 58.7    & 50.9    \\
\ours{ViT-H}     & \baseline{\bf 56.9} & \baseline{\bf 50.3} & \baseline{\bf 58.8} & \baseline{\bf 51.0} \\
\oursb{Hiera-H}   & \baseline{\bf 57.0} & \baseline{\bf 50.3} & \baseline{\bf 59.0} & \baseline{\bf 51.1} \\
\end{tabular}
    \captionof{table}{\textbf{COCO w/ Absolute Win.} Comparison between our ViTDet and HieraDet with absolute win and without. $^\ddagger$ Our implementation. }
    \label{tab:coco_backbones}

==> figures/16_coco_speed.tex <==

    \includegraphics[width=\linewidth]{figures/img/benchmark_box.png}\\
    \includegraphics[width=\linewidth]{figures/img/benchmark_mask.png}
    
    \captionof{figure}{\textbf{COCO Runtime.} Benchmarked on the same A100 using Mask R-CNN (fp16, bs=8).% In order: \citet{hiera,vitdet,mvit2,swin,simmim}.
    }
    \label{fig:coco_speed}

==> figures/17_coco_results.tex <==

    \centering
    \tablestyle{3pt}{1.08}
    \newcommand{\method}[1]{{\tiny #1}}
    \begin{tabular}{y{75}x{21}x{21}x{21}x{21}}
          & \multicolumn{2}{c}{\tiny single-scale test} & \multicolumn{2}{c}{\tiny multi-scale test} \\
    model & AP$^\text{box}$ & AP$^\text{mask}$ & AP$^\text{box}$ & AP$^\text{mask}$ \\\shline
    Swin-L \method{HTC++, 21K, sup} & 57.1 & 49.5 & 58.0 & 50.4 \\
    MViTv2-H \method{Cas, 21K, sup} & 57.1 & 48.8 & 58.4 & 50.1 \\
    CBNetV2 \method{HTC, 21K, sup} & 59.1 & 51.0 & 59.6 & 51.8 \\
    ViTDet-H \method{Cas, 1K, MAE} & {\underline{60.4}} & {\bf 52.0} & 61.3 & {\underline{53.1}} \\\hline
    \multicolumn{5}{c}{\baseline{\it \textbf{w/ absolute win}}}\\
    % ViTDet-H \method{Cas, 1K, MAE} & \\
    \baseline{{\bf Hiera-B} \method{Cas, 1K, MAE}} & \baseline{57.7} & \baseline{49.6} & \baseline{59.3} & \baseline{51.2} \\
    \baseline{{\bf Hiera-B+} \method{Cas, 1K, MAE}} & \baseline{58.5} & \baseline{50.4} & \baseline{60.0} & \baseline{52.0} \\
    \baseline{{\bf Hiera-L} \method{Cas, 1K, MAE}} & \baseline{60.1} & \baseline{51.6} & \baseline{\underline{61.5}} & \baseline{{53.0}}\\
    \baseline{{\bf Hiera-H} \method{Cas, 1K, MAE}} & \baseline{\bf 60.7} & \baseline{\bf{52.0}} & \baseline{\bf 61.7} & \baseline{\bf 53.3}\\
    \end{tabular}
    \captionof{table}{\textbf{COCO Results} on minival for methods pretrained on ImageNet \cite{swin,mvit2,cbnetv2,vitdet}. }
    \label{tab:coco_results}

==> figures/18_lvis_results.tex <==

    \centering
    \tablestyle{4pt}{1.08}
    \newcommand{\method}[1]{{\tiny #1}}
    \begin{tabular}{y{80}x{24}x{24}x{24}}
          & \multicolumn{3}{c}{\tiny single-scale test} \\
    model & AP$^\text{mask}$ & AP$^\text{mask}_\text{rare}$ & AP$^\text{box}$ \\\shline
    Detic \method{\citet{detic}} & 41.7 & \underline{41.7} & - \\
    CBNetV2$^\text{ 2021 Comp Winner}_\text{ \citet{lvischallengewinner}}$ & {\bf 49.2} & {\bf 45.4} & - \\
    ViTDet-L \method{\citet{vitdet}} & 46.0 & 34.3 & 51.2 \\ 
    ViTDet-H \method{\citet{vitdet}} & 48.1 & 36.9 & {\underline{53.4}} \\\hline
    \multicolumn{4}{c}{\baseline{\it \textbf{w/ absolute win}}}\\
    \baseline{{\bf Hiera-B} \method{abs win}} & \baseline{42.9} & \baseline{32.0} & \baseline{47.7} \\
    \baseline{{\bf Hiera-B+} \method{abs win}} & \baseline{43.9} & \baseline{30.7} & \baseline{48.9} \\
    \baseline{{\bf Hiera-L} \method{abs win}} & \baseline{47.1} & \baseline{37.4} & \baseline{52.5}\\
    \baseline{{\bf Hiera-H} \method{abs win}} & \baseline{\underline{48.9}} & \baseline{38.0} & \baseline{{\bf 54.6}}\\
    \end{tabular}
    \captionof{table}{\textbf{LVIS v1 Results.} System-level comparison using the same setup as \citet{vitdet}. }
    \label{tab:lvis_results}

==> figures/a5_sup_window_sim.tex <==
\begin{minipage}{0.48\linewidth}{
    \includegraphics[width=\linewidth]{figures/img/_sup_window_sim.png}
    
    \captionof{figure}{\textbf{Window Repetition} for \textit{fully supervised} baseline Hiera models on ImageNet-1k. Like Fig.~\ref{fig:window_sim}, but here showing both Hiera-B and Hiera-L models. Notably, the L model does not reach the same level of window similarity as B.  }
    \label{fig:sup_window_sim}
}\end{minipage}

==> figures/a6_sup_size_comparison.tex <==
\begin{minipage}{0.48\linewidth}{
\renewcommand{\good}[1]{\textcolor{good}{{+#1}}}
\newcommand{\ehh}[1]{\textcolor{gray}{{+#1}}}
\renewcommand{\bad}[1]{\textcolor{bad}{{-#1}}}
    \centering
    \tablestyle{4pt}{1.08}
    \begin{tabular}{y{45}y{48}x{28}x{20}}
        model    & pos embed & acc & $\Delta$ \\
        \shline
        Hiera-L$_{\text{Sup}}$ & absolute & 76.1 &  \\
                   & absolute win & \textbf{79.8} & \good{\bf 3.7}  \\
        \hline
        Hiera-B$_{\text{Sup}}$ & absolute & 81.8 &   \\
                   & absolute win & \textbf{82.4} & \good{\bf 0.6} \\
    \end{tabular}
    \captionof{table}{\textbf{Fully Supervised Training.} Absolute win can significantly improve the performance of a Hiera model trained from scratch. However, Hiera-L here benefits significantly more than Hiera-B. Fig.~\ref{fig:sup_window_sim} has a potential answer: Hiera-L doesn't learn the repeated window pattern.   }
    \label{tab:sup_size_comparison}
}\end{minipage}
